Adversarial Task Assignment

The problem of assigning tasks to workers is of long-standing fundamental importance. Examples of this include the classical problem of assigning computing tasks to nodes in a distributed computing environment, assigning jobs to robots, and crowdsourcing. Extensive research into this problem generally addresses important issues such as uncertainty and incentives. However, the problem of adversarial tampering with the task assignment process has not received as much attention. We are concerned with a particular adversarial setting where an attacker may target a set of workers in order to prevent the tasks assigned to these workers from being completed. When all tasks are homogeneous, we provide an efficient algorithm for computing the optimal assignment. When tasks are heterogeneous, we show that the adversarial assignment problem is NP-Hard, and present an algorithm for solving it approximately. Our theoretical results are accompanied by extensive experiments showing the effectiveness of our algorithms.

==> RandomizedLeaveOut.tex <==
\leaveout{
Given the pattern of the best allocation, we continue our analysis and look at the different environment parameters' role on the defender's expected utility. First, since the defender always assigns all the tasks to a single worker, we note that the number of tasks available, $ m $, will have no effect on the defender's expected utility per task. Thus, we only focus on the effect of the number of workers available to the defender ($ n $). Figure~\ref{fig:Randomized} visualizes this effect given two different distributions from which the workers' proficiencies were sampled: Uniform distribution and Power Law distribution (with $ k=0.5 $). Both distributions were truncated such that the sampled proficiency values are between $ 0.5 $ and $ 1 $. We setup multiple environments, all with $ 100 $ tasks where each of the environments differ by the number of workers ( $ 2 - 50 $ ). For each tuple of environment and distribution, we extract the defender's expected utility, averaged over $ 20,000 $ runs, each with a different workers' proficiencies.\footnote{For the case of $ i+1 $ workers, the same $ i $ workers as before were chosen along with one new worker.} Figure~\ref{subfig:randomizedutility} depicts the defender's expected utility when using randomized assignment given the different sampling distributions. Naturally, as the number of available workers increases, and thereby the number of assigned workers increases (as depicted in Figure~\ref{subfig:randomizedass}), the defender's expected utility increases as well. Especially, when workers' proficiencies were sampled from the Power Law distribution (i.e., with a larger portion of low proficient workers), we see that the expected utility is lower than the one using the Uniform distribution. The interesting insight is that in this case is that the defender also chooses to assign fewer workers as depicted in Figure~\ref{subfig:randomizedass}.%there is a decrease in the attack's efficiency that is represented in 
\begin{figure}[htb]
	\centering
	\begin{subfigure}{0.25\textwidth}
		\centering
		\resizebox{\height}{4cm}{
			\includegraphics[width=1.4\linewidth]{RandomizedUtil}
		}
		\caption{Expected utility}%Available workers' effect on the defender's expected utility}
		\label{subfig:randomizedutility}
	\end{subfigure}%
	\begin{subfigure}{0.25\textwidth}
		\centering
		\resizebox{\height}{4cm}{
		\includegraphics[width=1.4\linewidth]{RandomizedAss}
		}
		\caption{Assigned workers}
		\label{subfig:randomizedass}
	\end{subfigure}\hfil
	\caption{Randomized assignment}
	\label{fig:Randomized}
\end{figure}
}

\leaveout{
	\begin{figure}
		\begin{subfigure}{0.25\textwidth}
			\centering
			\resizebox{\height}{4cm}{
				\includegraphics[width=1.3\textwidth]{100tasks}
			}
			\caption{Expected utility} \label{fig:NumOfWorkers}
		\end{subfigure}%
		\begin{subfigure}{0.25\textwidth}
			\centering
			\resizebox{\height}{4cm}{
				\includegraphics[width=1.3\textwidth]{assignmentComp}}
			\caption{Assigned workers}
			\label{fig:assignmentcomp}
		\end{subfigure}
		\caption{Assignments' comparison}
	\end{figure}
	%As depicted in Figure~\ref{fig:NumOfWorkers}, even when the defender has the flexibility of not committing to a specific allocation, she will not result in a significant improvement in her expected utility. To further analyze the magnitude of possible improvement, we conduct a set of similar experiments, for environments with 20, 30, 50, 100 and 200 tasks while changing the number of workers from $ 2 $ to $ 10 $. For each tuple ($ m, n$), we extract the percentage of improvement by using Randomized assignment rather than a Deterministic one. 
	%As depicted in Figure~\ref{fig:ratio}, as the number of tasks increase, the improvement of using the Randomized assignment over the Deterministic one decreases, respectively. In a similar manner, as the number of workers increases, this improvement decreases as well.
	\begin{figure}
		\centering
		\resizebox{\height}{4cm}{
			\includegraphics[width=1.2\linewidth]{Ratio}
		}
		\caption{Improvement ratio - Randomized vs. Deterministic}
		\label{fig:ratio}
	\end{figure}
	%\begin{figure}
	%	\centering
	%	\includegraphics[width=0.45\textwidth]{assignmentComp}
	%	\caption{}
	%	\label{fig:assignmentcomp}
	%\end{figure}
	While the randomized assignment is promised to result in an higher expected utility, another factor to one should look at is the number of workers that are being assigned in each strategy. As depicted in Figure~\ref{fig:assignmentcomp}, which represents the number of assigned workers for our simulations using the Uniform distribution, the deterministic strategy results in assigning more workers in each case.
	\begin{figure}
		\centering
		\begin{subfigure}{0.25\textwidth}
			\centering
			\resizebox{\height}{4cm}{
				\includegraphics[width=1.4\textwidth]{5workers}
			}
			\caption{5 workers} \label{fig:5workers}
		\end{subfigure}%
		\begin{subfigure}{0.25\textwidth}
			\centering
			\resizebox{\height}{4cm}{
				\includegraphics[width=1.4\textwidth]{20workers}
			}
			\caption{20 workers}	\label{fig:20workers}
		\end{subfigure}
		\caption{The effect of tasks' availability on the defender's expected-utility} \label{fig:NumOfTasks}
	\end{figure}		
	Next, in Figure~\ref{fig:NumOfTasks}, we compare the per-task utility using the two strategies given different population sized: $ 5 $ workers (Figure~\ref{fig:5workers}) and $ 20 $  workers (Figure~\ref{fig:20workers}). For each case, we extract the defender's expected-utility when changing the number of available tasks from $ 20 $ to $ 50 $. As depicted in these figures, we observe a similar trend as in Figure~\ref{fig:NumOfWorkers}, that there is not much improvement by using the randomized strategy over the deterministic one.
}
